Temporal Graph ODEs for Irregularly-Sampled Time Series

Modern graph representation learning works mostly under the assumption of dealing with regularly sampled temporal graph snapshots, which is far from realistic, e.g., social networks and physical systems are characterized by continuous dynamics and sporadic observations. To address this limitation, we introduce the Temporal Graph Ordinary Differential Equation (TG-ODE) framework, which learns both the temporal and spatial dynamics from graph streams where the intervals between observations are not regularly spaced. We empirically validate the proposed approach on several graph benchmarks, showing that TG-ODE can achieve state-of-the-art performance in irregular graph stream tasks.

==> Sections/experiments_before25_5_2023.tex <==
\section{Experiments}
In this section, we discuss the empirical assessment of our method. Specifically, we first show the efficacy of handling dynamic graphs with irregularly sampled time series by evaluating our framework on several heat diffusion scenarios (see Section \ref{sec:heat_diffusion}). Afterwards, we assess the performance of the proposed approach on real graph benchmarks (see Section \ref{sec:real_bench}). The performance of our method is assessed against DGN variants from the literature. 
\revise{We carried the experiments on an cluster leveraging 7 out of 15 nodes (96 CPUs/node). We release openly the code implementing our methodology and reproducing our empirical analysis after acceptance. }%at: \revise{https://github.com/gravins/}.

\subsection{Heat diffusion}\label{sec:heat_diffusion}
\paragraph{Setup}
In the scenario of the heat diffusion tasks, the objective is to simulate the heat diffusion over a graph by leveraging irregularly sampled timestamps. Thus, we predict the future temperature of each node in the given graph given the irregular history of temperatures. More formally, $$\mathbf{X}_{t+\Delta t} = \arg\max \mathbb{P}(\mathbf{X}_{t+\Delta t} | \mathbf{X}_{1}, ...\, , \mathbf{X}_{t}),$$ where $\Delta t$ is irregular over the time series. 

In our experiment, we leveraged a grid graph consisting of 70 nodes in which each node is characterized by an initial temperature, which is randomly sampled in the range between $0$ and $0.2$. We considered two different settings for our experiments. In the first experimental scenario, we randomly select a node and increase its initial temperature to a value between $10$ and $15$ (\ie we generate a hot spike). In the second scenario, we randomly alter the initial temperature of a third of the nodes by generating a hot or cold spike. A cold spike is characterized by a temperature between $-15$ and $-10$, and it has a probability of $0.4$ to occur. 
We collected the ground truth by simulating the heat diffusion equation through the forward Euler's method with a step size, $\epsilon$, equal to $10^{-3}$. We illustrate the simulation of the heat diffusion in Figure~\ref{fig:heat_diffusion}.


\begin{figure*}[h]
    \centering
    \subfloat[]{\includegraphics[width=0.4\textwidth]{Images/head_diffusion_0steps.png}}
    \hspace{1cm}
    \subfloat[]{\includegraphics[width=0.4\textwidth]{Images/head_diffusion_1000steps.png}}
    \caption{(a) A grid graph consisting of 70 nodes in which each node is characterized by an initial temperature. To darker colors corresponds colder temperatures, while brighter colors mean warmer temperatures. (b) The heat diffusion simulation computed through 1000 steps forward Euler's method. The simulation is computed leveraging $-\mathbf{L}\mathbf{X}(t)$ as diffusion equation.}
    \label{fig:heat_diffusion}
\end{figure*}

The training set consists of 100 randomly selected timestamps over the 1000 steps used to simulate the diffusion process. The validation and test sets are generated from two different simulations similar to the one used for building the training set. However, these sets are obtained through 500 steps simulations, and only 50 of them are kept as validation/test set. We simulated seven different diffusion functions, \ie $-\mathbf{L}\mathbf{X}(t)$, $-\mathbf{L}^2\mathbf{X}(t)$, $-\mathbf{L}^5\mathbf{X}(t)$, $-\tanh(\mathbf{L})\mathbf{X}(t)$, $-5\mathbf{L}\mathbf{X}(t)$, $-0.05\mathbf{L}\mathbf{X}(t)$, and $-(\mathbf{L}+\mathcal{N}_{0,1})\mathbf{X}(t)$. Here, $\mathcal{N}_{0,1}$ stands for a noise sampled from a standard normal distribution, and $\mathbf{L}$ is the normalized graph Laplacian. 

We explored the performance of our framework, \method{}, by leveraging the aggregation scheme proposed in \cite{tagcn} and forward Euler's method as discretization procedure, for simplicity. Thus, the nodes' states for the entire snapshot are updated as
\begin{equation}
        \mathbf{X}^\ell = \mathbf{X}^{\ell-1} +\epsilon\sigma\left(\sum_{k=0}^K \mathbf{L}^k \mathbf{X}^{\ell-1} \mathbf{W}_{k}\right),
\end{equation}
where $K$ corresponds to the number of filters and $\mathbf{W}_{k}$ is the $k$-th weight matrix.
We recall that other choices of aggregation and discretization schemes are possible. We compared our method with five common DGNs for dynamic graphs. Specifically,
\begin{itemize}
    \item \textbf{DCRNN} a recurrent graph network presented in \cite{DCRNN};
    \item \textbf{TGCN} the temporal Graph Convolutional Network presented in \cite{TGCN}
    \item \textbf{A3TGCN} the attentive architecture based on TGCN from \cite{a3tgcn}; 
    \item \textbf{GCRN-GRU} a generalization of the classical gated recurrent unit to graph data presented in \cite{GCRN};
    \item \textbf{GCRN-LSTM} the architecture that stacks an LSTM on top of the DGN computation presented in \cite{GCRN}.
\end{itemize}

We designed each model as a combination of three main components. The first is the encoder which maps the node input features into a latent hidden space; the second is the temporal graph convolution (\ie, \method{} or the DGN baselines); and the third is a readout that maps the output of the convolution into the output space. The encoder and the readout are Multi-Layer Perceptrons that share the same architecture among all models in the experiments.

To allow the baselines to deal with irregular timestamps, we used a similar strategy employed by \method{}. Specifically, we selected the unit of time, $\tau$,  and then we iteratively applied the temporal graph convolution for a number of steps equal to the ration between the time difference between two consecutive timestamps and the time unit, \ie $\#steps = (t_i -t_{i+1})/ \tau$. 

We performed hyper-parameter tuning via grid search, optimizing the Mean Absolute Error (MAE). We trained the models using Adam optimizer for a maximum of 3000 epochs and early stopping with patience of 100 epochs on the validation error. In Table~\ref{tab:configs_heat} we report the grids of hyper-parameters employed in our heat diffusion experiments by each method. We recall that the hyper-parameter $\epsilon$ refers only to our method, and that embedding dim equal to None means that no encoder and readout are employed.
\input{Tables/conf_heat_diff.tex}


\paragraph{Results}
\revise{TODO} We present the results on the heat diffusion tasks with one initial spike in Table~\ref{tab:single_spike}. Specifically, we report the $log_{10}(\mathrm{MAE})$ as evaluation metric. The firs observation is that \method{} has outstanding compared to the baselines employed in the experiment. Indeed, our method produce an error that is several order of magnitude lower that the best baseline in each task.  


In Table~\ref{tab:multi_spike} we present the scenario with multiple initial spikes. Specifically, we report the $log_{10}(\mathrm{MAE})$ as evaluation metric. We observe that our method outperforms the selected baselines on all tasks. Indeed, \method{} achieves a performance that is 30\% to 1060\% better than the best baseline in each task in the first scenario. Notably, the performance gap is increased in the scenario with multiple initial spikes, where \method{} is up to 1310\% better than the best baseline. 
\input{Tables/heat_uno_spike.tex}
\input{Tables/heat_molti_spike.tex}

\subsection{Graph Benchmarks}\label{sec:real_bench}

\paragraph{Setup}
In the scenario of the graph benchmarks, the objective is to perform traffic forecasting leveraging irregular time series. Thus, similarly to the heat diffusion tasks we predict the future node values given the past history.

We considered five real world graph benchmark for traffic forecasting. The first kind of datasets are about highway  traffic information in California. collect by  
\begin{itemize}
    \item \textbf{MetrLA}~\cite{DCRNN}: four months of traffic information, aggregated in 5 minutes intervals, collected from 207 loop detectors in the highway of Los Angeles County;
    \item \textbf{Montevideo}~\cite{rozemberczki2021pytorch}: one month of hourly passenger inflow at bus stop level for eleven bus lines from the city of Montevideo;
    \item \textbf{PeMS03}~\cite{pems03-08}: three months of traffic readings collected every 5 minutes from 358 traffic sensors by California Transportation Agencies (CalTrans) Performance Measurement System (PeMS);
    \item \textbf{PeMS04}~\cite{pems03-08}: two months of 307 traffic sensorss readings, aggregated into 5-minute intervals, collected by the CalTrans PeMS in the San Francisco Bay Area ;
    \item \textbf{PeMS07}~\cite{pems03-08}: four months of of traffic readings collected every 5 minutes from 883 traffic sensors by the CalTrans PeMS;
    \item \textbf{PeMS08}~\cite{pems03-08}: two months of 170 traffic sensors readings, aggregated into 5-minute intervals, by the CalTrans PeMS in San Bernardino.
\end{itemize} 
We report additional details about the datasets in Table~\ref{tab:graph_benchmark_stats}. Since we used a modified version of the original datasets (\ie we employed irregular timestamps), we will refer to the datasets by using the subscript $i$ to make clear the difference from the original version.

\input{Tables/traffic_dataset_stats}


We generated the irregular time series by randomly selecting a third of the original graph snapshots. We considered a temporal data splitting in which 80\% of the previously selected snapshots are used as training set, 10\% as validation set and the remaining as test set.

Also for this class of experiments, we considered the same baselines and architectural choices as for the heat diffusion experiments. Even in this scenario, we performed hyper-parameter tuning via grid search, optimizing the Mean Absolute Error (MAE). We trained the models using Adam optimizer for a maximum of 3000 epochs and early stopping with patience of 100 epochs on the validation error. In Table~\ref{tab:configs_traffic} we report the grids of hyper-parameters employed in our heat diffusion experiments by each method. We recall that the hyper-parameter $\epsilon$ refers only to our method.
\input{Tables/conf_traffic}


\paragraph{Results}
\revise{TODO}
\input{Tables/traffic.tex}
\input{Tables/traffic_time}


==> Tables/ablation_pems04.tex <==
%\renewcommand{\arraystretch}{1.3}
\begin{table*}[h!]
\centering
\caption{Test $\mathrm{MAE}$ scores and std of TG-ODE on PeMS04, averaged over 5 runs, for dataset sizes of 500, 1000, 2000, 4000, 8000, and 16000 randomly sampled samples.}\label{tab:ablation}
\small
\begin{tabular}{cccccc}
\hline\toprule%\hline

\textbf{500}       & \textbf{1000}       & \textbf{2000}       & \textbf{4000}        & \textbf{8000}       & \textbf{16000} \\ \midrule%\hline 
67.31$_{\pm0.374}$ & 48.023$_{\pm0.045}$ & 34.761$_{\pm0.049}$ & 27.946$_{\pm0.131}$  & 22.777$_{\pm0.014}$ & 20.838$_{\pm0.012}$     \\\bottomrule\hline%\hline

%Our         & 67.31022796630859$_{\pm0.374092349447039}$ & 48.022987365722656$_{\pm0.04533229421999933}$ & 34.760649871826175$_{\pm0.04893570322757043}$ & 27.946232986450195$_{\pm0.130984615800167}$ & 22.776685333251955$_{\pm0.014157688474605927}$ & 20.837573623657228$_{\pm0.01167331554186364}$


\end{tabular}
\end{table*}



==> Tables/conf_heat_diff.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.3}
\caption{The grid of hyper-parameters employed during model selection for the heat diffusion tasks.\label{tab:configs_heat}}
\small
\centering
\begin{tabular}{ll}
\hline\hline
 & \textbf{Configs}\\\hline
learning rate & $10^{-2}$, $10^{-3}$, $10^{-4}$\\
weight decay &  $10^{-2}$, $10^{-3}$\\
$\psi$ & concat, sum, $\psi(\overline{\mathbf x}, \hat{\mathbf x})=\overline{\mathbf x}$\\
activ fun & tanh, relu, identity\\
embedding dim & None, 8\\
$\epsilon$ & $10^{-3}$\\
\# hops & 5\\\hline\hline
%Chebyshev filter size & 5\\\hline\hline
\end{tabular}
\end{table}

==> Tables/conf_traffic.tex <==
\begin{table}[h]
\renewcommand{\arraystretch}{1.3}
\caption{The grid of hyper-parameters employed during model selection for the graph benchmarks tasks.\label{tab:configs_traffic}}
\small
\centering
\begin{tabular}{ll}
\hline\hline
 & \textbf{Configs}\\\hline
learning rate & $10^{-2}$, $10^{-3}$, $10^{-4}$\\
weight decay &  $10^{-2}$, $10^{-3}$\\
$\psi$ & concat, sum, $\psi(\overline{\mathbf x}, \hat{\mathbf x})=\overline{\mathbf x}$\\
activ fun & tanh, relu, identity\\
embedding dim & 64, 32\\
$\epsilon$ & 1, 0.5, $10^{-1}$, $10^{-2}$, $10^{-3}$\\
\# hops & 1, 2, 5\\\hline\hline
%Chebyshev filter size & 1, 2, 5\\\hline\hline
\end{tabular}
\end{table}

==> Tables/traffic_time.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table*}[h!]
\centering
\caption{Average time per epoch (measured in seconds) and std computed leveraging an Intel Xeon Gold 6240R CPU @ 2.40GHz. Each time is obtained employing 5 neighbor hops and embedding dimension equal to 64.}\label{tab:timing}
\small
\begin{tabular}{lcccccc}
\hline\hline
   & \textbf{MetrLA$_i$}   & \textbf{Montevideo$_i$}    & \textbf{PeMS03$_i$}            & \textbf{PeMS04$_i$}           & \textbf{PeMS07$_i$}     & \textbf{PeMS08$_i$}   \\  \hline
A3TGCN    & 261.32$_{\pm24.55}$   & 9.09$_{\pm0.49}$  & 226.00$_{\pm54.26}$   & 146.18$_{\pm54.07}$  & 581.14$_{\pm397.50}$  & 173.97$_{\pm82.55}$ \\  
DCRNN     & 1394.24$_{\pm139.02}$ & 45.41$_{\pm0.97}$ & 762.65$_{\pm87.91}$   & 485.02$_{\pm108.93}$ & 1713.95$_{\pm2.01}$   & 393.21$_{\pm49.62}$ \\  
GCRN-GRU  & 1112.56$_{\pm181.01}$ & 51.64$_{\pm0.92}$ & 749.48$_{\pm93.01}$   & 465.60$_{\pm91.55}$  & 1517.17$_{\pm87.55}$   & 425.52$_{\pm52.80}$ \\  
GCRN-LSTM & 1433.74$_{\pm175.29}$ & 58.86$_{\pm3.02}$ & 1005.78$_{\pm158.74}$ & 605.01$_{\pm98.08}$  & 1973.41$_{\pm231.04}$ & 541.63$_{\pm79.92}$ \\ 

% \rowcolor{red}
% NDCN              & 63.06$_{\pm0.55}$ & 1.46$_{\pm0.03}$ & 38.32$_{\pm0.79}$ & 24.79$_{\pm0.29}$ & 64.05$_{\pm1.6}$ & 21.11$_{\pm0.38}$\\
% \rowcolor{red}
NDCN%$_{torchdyn}$ 
& \textbf{159.42$_{\pm2.62}$} & \textbf{3.79$_{\pm0.09}$} & \textbf{108.93$_{\pm1.7}$} & \textbf{70.68$_{\pm0.94}$} & \textbf{146.09$_{\pm2.05}$} & \textbf{62.72$_{\pm0.5}$}\\
% \rowcolor{red}
% NODE              & 25.14$_{\pm0.41}$ & 0.99$_{\pm0.02}$ & 21.95$_{\pm0.4}$ & 13.97$_{\pm0.42}$ & 37.86$_{\pm0.59}$ & 13.39$_{\pm0.31}$\\
% \rowcolor{red}
% NODE$_{torchdyn}$ & 57.35$_{\pm0.55}$ & 2.06$_{\pm0.04}$ & 51.11$_{\pm0.29}$ & 33.25$_{\pm0.68}$ & 79.95$_{\pm1.14}$ & 31.76$_{\pm0.57}$\\

TGCN      & 267.42$_{\pm39.97}$   & 9.09$_{\pm0.10}$  & 209.86$_{\pm46.16}$   & 159.38$_{\pm60.21}$  & 575.89$_{\pm395.12}$  & 170.07$_{\pm83.38}$ \vspace{0.1cm}\\  
Our       & \textbf{231.17$_{\pm39.14}$}   & \textbf{4.48$_{\pm0.35}$}  & \textbf{136.94$_{\pm2.05}$}    & \textbf{72.44$_{\pm2.86}$}    & \textbf{194.26$_{\pm20.64}$}   & \textbf{64.32$_{\pm1.30}$}   \\  \hline\hline

%                &\textbf{DCRNN}         & \textbf{GCRN-GRU}     & \textbf{GCRN-LSTM}    & \textbf{A3TGCN}      & \textbf{TGCN}        &    \textbf{Our}      \\\hline 
% MetrLA$_i$     & 1394.24\tiny{$_{\pm139.02}$} & 1112.56$_{\pm181.01}$ & 1433.74$_{\pm175.29}$ &  261.32$_{\pm24.55}$ &  267.42$_{\pm39.97}$ &  231.17$_{\pm39.14}$ \\
% Montevideo$_i$ &     45.41$_{\pm0.97}$ &     51.64$_{\pm0.92}$ &     58.86$_{\pm3.02}$ &     9.09$_{\pm0.49}$ &     9.09$_{\pm0.10}$ &     4.48$_{\pm0.35}$ \\
% PeMS03$_i$     &   762.65$_{\pm87.91}$ &   749.48$_{\pm93.01}$ & 1005.78$_{\pm158.74}$ &  226.00$_{\pm54.26}$ &  209.86$_{\pm46.16}$ &   136.94$_{\pm2.05}$ \\
% PeMS04$_i$     &  485.02$_{\pm108.93}$ &   465.60$_{\pm91.55}$ &   605.01$_{\pm98.08}$ &  146.18$_{\pm54.07}$ &  159.38$_{\pm60.21}$ &    72.44$_{\pm2.86}$ \\
% PeMS07$_i$     &   1713.95$_{\pm2.01}$ &   68.83$_{\pm258.99}$ & 1973.41$_{\pm231.04}$ & 581.14$_{\pm397.50}$ & 575.89$_{\pm395.12}$ &  194.26$_{\pm20.64}$ \\
% PeMS08$_i$     &   393.21$_{\pm49.62}$ &   425.52$_{\pm52.80}$ &   541.63$_{\pm79.92}$ &  173.97$_{\pm82.55}$ &  170.07$_{\pm83.38}$ &    64.32$_{\pm1.30}$ \\\hline\hline
\end{tabular}
\end{table*}
